Graph Generation with $K^2$-trees

Generating graphs from a target distribution is a significant challenge across many domains, including drug discovery and social network analysis. In this work, we introduce a novel graph generation method leveraging $K^2$-tree representation, originally designed for lossless graph compression. The $K^2$-tree representation {encompasses inherent hierarchy while enabling compact graph generation}. In addition, we make contributions by (1) presenting a sequential $K^2$-treerepresentation that incorporates pruning, flattening, and tokenization processes and (2) introducing a Transformer-based architecture designed to generate the sequence by incorporating a specialized tree positional encoding scheme. Finally, we extensively evaluate our algorithm on four general and two molecular graph datasets to confirm its superiority for graph generation.

==> algorithm/algo_pre_post.tex <==
%\setlength{\intextsep}{0pt}%
%\setlength{\columnsep}{11pt}%
%\begin{wrapfigure}{R}{0.6\textwidth}
%\begin{minipage}[t]{\linewidth}
\begin{algorithm}[t]
\caption{Finding prefixes and postfixes of redundant nodes in \tree}
\label{algo:pre_post}
\begin{algorithmic}
\Statex \textbf{Input}: $k$
\Statex \textbf{Output}: two lists of prefixes and postfixes
\Statex Prefixes = []
\Statex Postfixes = []
\For{$i \gets 1 \text{ to } k$} \Comment{To update prefixes (diagonal indices of $k^2$ cells)}
    \State $\text{idx}= (i-1)*k+i$
    \State Prefixes.append(idx)
\EndFor
\For{$i \gets 1 \text{ to } k-1$} \Comment{To update postfixes (upper diagonal indices of $k^2$ cells)}
\For{$j \gets i+1 \text{ to } k$}
    \State $\text{idx}= (j-1)*k+j$
    \State Postfixes.append(idx)
\EndFor
\EndFor
\end{algorithmic}
\end{algorithm}
%\end{minipage}
%\end{wrapfigure}

==> algorithm/algo_red.tex <==
%\setlength{\intextsep}{0pt}%
%\setlength{\columnsep}{11pt}%
%\begin{wrapfigure}{R}{0.6\textwidth}
%\begin{minipage}[t]{\linewidth}
\begin{algorithm}[H]
\caption{Deciding redundancy of a tree node in \tree}
\label{algo:redundancy}
\begin{algorithmic}
\Statex \textbf{Input}: a tree node $t \in T$ with position $[p_1, p_2, \dots, p_h]$
\Statex Prefixes = $[{pr}_1, {pr}_2, \dots, {pr}_k]$
\Statex Postfixes = $[{po}_1, {po}_2, ..., {po}_{\frac{(k-1)(k-2)}{2}}]$
\If{${p_1, p_2, \dots, p_{h-1}} \in  \text{prefixes}$ and $p_h \in \text{postfixes}$}
    \State  \Return true
\Else
    \State \Return false
\EndIf
\end{algorithmic}
\end{algorithm}
%\end{minipage}
%\end{wrapfigure}

==> algorithm/algo_seqtok2.tex <==
\begin{wrapfigure}{r}{0.63\textwidth}
\begin{minipage}{0.63\textwidth}
\begin{algorithm}[H]
\caption{\tree construction from sequence $\bm{y}$}\label{alg:seqtok2}
\label{algo:k2tree}
\begin{algorithmic}[1]
\State \textbf{Input}: Sequential representation $\bm{y}=y_{1},\ldots, y_{T}$.
\State Initialize a tree $T=(\{r\}, \emptyset)$
\State Initialize a queue $\mathcal{Q}=[r]$
\While{$Q \neq \emptyset$}
\State Pop $u$ from $\mathcal{Q}$
\ForEach{$y_t = (x_1, \ldots, x_?) \in \bm{y}$}
    \ForEach{$x \in y_t$}
    \State Add child tree-node $v$ where $x_v=x$ to $u \in T$
    \If{$x=1$ and $|A^{(v)}|>(1\times 1)$}
    \State Insert $x$ in $\mathcal{Q}$
    \EndIf    
    \EndFor

\EndFor
\EndWhile
\State Step 1. 
\State Step 2.
\end{algorithmic}
\end{algorithm}
\end{minipage}
\end{wrapfigure}


==> algorithm/algo_treepe.tex <==
\begin{algorithm}
\caption{Tree positional encoding in \tree}
\label{algo:tree_pe}
\begin{algorithmic}
\Statex \textbf{Input}: $t=(p(t), o) \in T$ \Comment{$p(t)$: parent tree node, $o$: order between sibling nodes}
\Statex \textbf{Output}: $PE(t)$ \Comment{tree positional encoding of $t$}

\If {$t$ is root}
    \State \Return 1
\Else
    \State \Return $PE(p(t))||o$ \Comment{Concatenate PE of parent node and order}
\EndIf

\end{algorithmic}
\end{algorithm}

==> figure/fig_ab_pe.tex <==
% \begin{wrapfigure}{r}{0.4\textwidth}
% \centering
% \vspace{-.1in}
% \includegraphics[width=.8\linewidth]{figure/ab_pe_loss.png}
%     \caption{Train curve for different PEs.}
%     \vspace{-.1in}
%   \label{fig:ab_pe}
% \end{wrapfigure}


==> table/tab_ab_comp.tex <==
% \begin{wraptable}{r}{0.4\textwidth}
% %\begin{table}
% % \vspace{-.1in}
%   \caption{Compression ratio on orderings.}\label{tab:ab_compression}
%   \centering
%   \scalebox{0.8}{
%     \begin{tabular}{lcccc}
%     % \toprule & Ego-small & Community-small & Enzymes & Grid & Planar & SBM & Proteins \\
%     \toprule 
%     Method & Comm. & Planar & Enzymes & Grid \\
%     \midrule
%     BFS  & 0.534 & 0.201 & 0.432 & 0.048 \\
%     DFS & 0.619 & 0.204 & 0.523 & 0.064 \\
%     C-M & \textbf{0.508} & \textbf{0.195} & \textbf{0.404} & \textbf{0.045} \\
%     \bottomrule
%   \end{tabular}
%   }

% %\end{table}
% \end{wraptable}
